Partial Key Grouping: Load-Balanced Partitioning of Distributed Streams

We study the problem of load balancing in distributed stream processing engines, which is exacerbated in the presence of skew. We introduce Partial Key Grouping (PKG), a new stream partitioning scheme that adapts the classical "power of two choices" to a distributed streaming setting by leveraging two novel techniques: key splitting and local load estimation. In so doing, it achieves better load balancing than key grouping while being more scalable than shuffle grouping. We test PKG on several large datasets, both real-world and synthetic. Compared to standard hashing, PKG reduces the load imbalance by up to several orders of magnitude, and often achieves nearly-perfect load balance. This result translates into an improvement of up to 175% in throughput and up to 45% in latency when deployed on a real Storm cluster. PKG has been integrated in Apache Storm v0.10.

==> README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society journal subset of the full
IEEEtran package and is intended for use with Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_jrnl_compsoc.tex.
***************************************************************************


==> notes.tex <==
% !TEX root =  ../main.tex
\section{Notes}
\begin{enumerate}
\item Load balancing in streams is an important issue when input distribution of keys is skewed
\begin{enumerate}
\item Current solutions do not work for different reasons (key grouping, shuffle grouping)
\item Hasn’t been studied well so far
\item Setting is Storm-like (no key identity in PE, no key migration possible)
\end{enumerate}
\item We propose to use PoTC to address the issue (nothing new here)
\begin{enumerate}
\item PoTC with “sticky” key grouping would give already good results (David’s simulations + proofs)
\item However PoTC can’t be used out of the box with multiple sources because there is a coordination problem (need to remember and have consensus on which of the choices is taken)
\end{enumerate}
\item We propose partial key grouping (``key splitting'') to address this issue (needs additional merge phase like shuffle grouping)
\begin{enumerate}
\item This requires a slightly different programming paradigm, which however has many applications (word count, naive bayes, sketches, SPDT)
\item We show that it works even better than normal PoTC (proof? and simulations)
\item Does not require coordination among sources (but requires load estimation)
\end{enumerate}
\item We propose local load estimation at the sources in a practical scenario
\begin{enumerate}
\item Compare with omniscient oracle (simulations)
\item Assess if some lightweight form of communication with destinations is useful (?) (simulations?)
\end{enumerate}
\item If the number of destinations/bins B are too many the load is unbalanced anyway
\begin{enumerate}
\item Key splitting helps in this case (explore power of d choices for $d>2$)
\end{enumerate}
\item We modify Storm to implement partial key grouping
\begin{enumerate}
\item Tests on live system
\item Release code
\end{enumerate}
\end{enumerate}

\section{Naming Conventions}

\begin{table}[htdp]
\caption{default}
\begin{center}
\begin{tabular}{l p{0.7\columnwidth}}
Partition		&	a division of the stream into sub-streams \\
Grouping		&	see Partition \\
Sub-Stream	&	a portion of the stream created by a partition \\
Message		&	an element of a stream, composed by a Key-Value pair \\
Tuple		&	see Message \\
Key			&	part of a Message that represents its identity \\
Stream		&	an infinite sequence of keyed messages \\
Key splitting	&	assigning a key to multiple (2) \peis \\
Power of both choices	&	see Key splitting \\
Static \potc	&	power of two choices \emph{without} key splitting \\
\end{tabular}
\end{center}
\label{default}
\end{table}%

